From Robot Self-Localization to Global-Localization: An RSSI Based Approach

Localization is a crucial task for autonomous mobile robots in order to successfully move to goal locations in their environment. Usually, this is done in a robot-centric manner, where the robot maintains a map with its body in the center. In swarm robotics applications, where a group of robots needs to coordinate in order to achieve their common goals, robot-centric localization will not suffice as each member of the swarm has its own frame of reference. One way to deal with this problem is to create, maintain and share a common map (global coordinate system), among the members of the swarm. This paper presents an approach to global localization for a group of robots in unknown, GPS and landmark free environments that extends the localization scheme of the LadyBug algorithm. The main idea relies on members of the swarm staying still and acting as beacons, emitting electromagnetic signals. These stationary robots form a global frame of reference and the rest of the group localize themselves in it using the Received Signal Strength Indicator (RSSI). The proposed method is evaluated, and the results obtained from the experiments are promising.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{A. Ferrando, R.C. Cardoso (Eds.): Third Workshop on\\ Agents and Robots for reliable Engineered Autonomy 2023 (AREA'23)\\
EPTCS 391, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.391.4}{10.4204/EPTCS.391.4}}

